On Computing Probabilistic Abductive Explanations

The most widely studied explainable AI (XAI) approaches are unsound. This is the case with well-known model-agnostic explanation approaches, and it is also the case with approaches based on saliency maps. One solution is to consider intrinsic interpretability, which does not exhibit the drawback of unsoundness. Unfortunately, intrinsic interpretability can display unwieldy explanation redundancy. Formal explainability represents the alternative to these non-rigorous approaches, with one example being PI-explanations. Unfortunately, PI-explanations also exhibit important drawbacks, the most visible of which is arguably their size. Recently, it has been observed that the (absolute) rigor of PI-explanations can be traded off for a smaller explanation size, by computing the so-called relevant sets. Given some positive {\delta}, a set S of features is {\delta}-relevant if, when the features in S are fixed, the probability of getting the target class exceeds {\delta}. However, even for very simple classifiers, the complexity of computing relevant sets of features is prohibitive, with the decision problem being NPPP-complete for circuit-based classifiers. In contrast with earlier negative results, this paper investigates practical approaches for computing relevant sets for a number of widely used classifiers that include Decision Trees (DTs), Naive Bayes Classifiers (NBCs), and several families of classifiers obtained from propositional languages. Moreover, the paper shows that, in practice, and for these families of classifiers, relevant sets are easy to compute. Furthermore, the experiments confirm that succinct sets of relevant features can be obtained for the families of classifiers considered.

==> algs/apaxp.tex <==
\begin{flushleft}
\hspace*{\algorithmicindent}
\textbf{Input}: {Classifier $\kappa$, instance $\mbf{v}$, threshold $\delta$}\\
\hspace*{\algorithmicindent}
\textbf{Output}: { $\apaxp~~\fml{S}$}
  %
\end{flushleft}
%
\begin{algorithmic}[1]
  \Procedure{$\apaxp$}{$\kappa,\mbf{v}, \delta$}
  \State{$\fml{S} \gets \{1,\ldots,m\}$}
  \For{$i\in\{1,\ldots,m\}$}
    \If{$\isweakpaxp(\fml{S}\setminus\{i\}, \kappa(\mbf{x})=c, \delta)$}
      \State{$\fml{S} \gets \fml{S}\setminus\{i\}$}
    \EndIf
  \EndFor  
  \State{\bfseries{return}~{$\fml{S}$}}
\EndProcedure
\end{algorithmic}

==> algs/paxpalgo.tex <==
\begin{flushleft}
\hspace*{\algorithmicindent}
\textbf{Input}: {Features $\{1,\ldots,m\}$; feature space
  $\mbb{F}$, classifier $\kappa$, instance $(\mbf{v},c)$, threshold
  $\delta$}\\ 
\hspace*{\algorithmicindent}
\textbf{Output}: {PAXp $\fml{S}$}
%
\end{flushleft}
%
\begin{algorithmic}[2]
  \Procedure{$\findpaxp$}{$\{1,\dots,m\};\mbb{F},\kappa,\mbf{v},c,\delta$}
  \State{$\fml{S} \gets \{1,\ldots,m\}$}
  \For{$i\in\{1,\ldots,m\}$}
    \If{$\issupersetpaxp(\fml{S}\setminus\{i\};\mbb{F},\kappa,\mbf{v},c,\delta)$}
      \State{$\fml{S} \gets \fml{S}\setminus\{i\}$}
    \EndIf
  \EndFor  
  \State{\bfseries{return}~{$\fml{S}$}}
\EndProcedure
\end{algorithmic}


==> tabs/dt/nouse.tex <==

\begin{comment}
%
%
%\begin{table}[t]
%\begin{adjustbox}{angle=90}
%\rotatebox{90}{
%\vbox{
\begin{sidewaystable}
  \centering
  \caption{ToDo}
  \renewcommand{\arraystretch}{1.15}
  \renewcommand{\tabcolsep}{0.425em}
  \begin{tabular}{c|cccc|cccc|cc|cc} \toprule
    Path & \multicolumn{10}{|c|}{Features \& Values} & $\eta_{jk}$ & $\eta_{mk}$ \\
    \cline{2-11}
    & \multicolumn{4}{|c|}{1} & \multicolumn{4}{|c|}{2} &
    \multicolumn{2}{|c|}{3} \\
    \cline{2-11}
    & 1 & 2 & 3 & 4 & 1 & 2 & 3 & 4 & 1 & 2    
    \\ \toprule
    $R_1$ &
    $s_{1,1,1}=s_{1,0,1}+\ite(u_1,\eta_{0,1},0)$ &
    $s_{1,2,1}=s_{1,1,1}$ &
    $s_{1,3,1}=s_{1,2,1}$ &
    $s_{1,4,1}=s_{1,3,1}$ &
    %$\eta_{11}=$
    %
    $s_{2,1,1}=s_{2,0,1}$ &
    $s_{2,2,1}=s_{2,1,1}+\ite(u_2,\eta_{0,1},0)$ &
    &
    &
    %
    &
    &  
    \\
    $R_2$ & & & & & & & & & & &  
    \\
    $R_3$ & & & & & & & & & & &  
    \\
    $R_4$ & & & & & & & & & & &  
    \\
    $R_5$ & & & & & & & & & & &  
    \\
    \bottomrule
  \end{tabular}
\end{sidewaystable}
%}
%}
%\caption{ToDo}
%\end{adjustbox}
%\end{table}
%
%
\end{comment}

\begin{comment}
%
%
\begin{table}[t]
  \centering
  \renewcommand{\arraystretch}{1.15}
  \renewcommand{\tabcolsep}{0.225em}
  \scalebox{0.9}{
    %{\smaller{%\smaller
      \begin{tabular}{c|C{2.75cm}C{2.75cm}C{2.75cm}C{2.75cm}|c} \toprule
        \multirow{3}{*}{Path}
        & \multicolumn{4}{c|}{Feature \& Values} &
        \multirow{3}{*}{$\eta_{jk}$} \\
        \cline{2-5}
        & \multicolumn{4}{c|}{$j=1$} \\
        \cline{2-5}
        & $s_{j,1,k}$ & $s_{j,2,k}$ & $s_{j,3,k}$ & $s_{j,4,k}$ &
        \\ \toprule
        %
        $R_1$ &
        $s_{1,0,1}+\ite(u_1,\eta_{0,1},0)$ &
        $s_{1,1,1}$ &
        $s_{1,2,1}$ &
        $s_{1,3,1}$ &
        $s_{1,4,1}$ \\
        %
        $R_2$ &
        $s_{1,0,1}+\ite(u_1,\eta_{0,1},0)$ &
        $s_{1,1,1}$ &
        $s_{1,2,1}$ &
        $s_{1,3,1}$ &
        $s_{1,4,1}$ \\
        %
        \bottomrule
        %
      \end{tabular}
    %}}
  }
  \caption{ToDo}
\end{table}
%
%
\end{comment}


==> tabs/dt/paxp-res.tex <==
\setlength{\tabcolsep}{4pt}
\let\lpr\undefined
\let\rpr\undefined
\newcommand{\lpr}{(}
\newcommand{\rpr}{)}

\sisetup{%
  math-rm=\textrm
}

\begin{table*}[bp]
\centering
\resizebox{0.75\textwidth}{!}{
  \begin{tabular}{l  S[table-format=3] c  S[table-format=3]  ccS[table-format=2.2]    ccS[table-format=1.2]  }
\toprule[1.2pt]
\multirow{2}{*}{\bf Dataset} &   & {\bf Path}  &   & \multicolumn{3}{c}{$\bm\mdrset$} & \multicolumn{3}{c}{$\bm\adrset$} \\
\cmidrule[0.8pt](lr{.75em}){3-3}
\cmidrule[0.8pt](lr{.75em}){5-7}
\cmidrule[0.8pt](lr{.75em}){8-10}
  & {\bf \#I} & {\bf Length} & {$\bm\delta$ } & {\bf Length} & {\bf Precision} & {\bf Time} &  {\bf Length} & {\bf Precision} &{\bf Time} \\  

\toprule[1.2pt]

%
 &  &  & 100 & 8.2 $\pm$ 0.5 & 100 & 5.84 & 8.2 $\pm$ 0.5 & 100 & 1.24  \\
adult & 160 & 12.3 $\pm$ 1.4 & 95 & 7.3 $\pm$ 1.1 & 97.7 & 35.19 & 7.5 $\pm$ 0.9 & 98.0 & 0.01  \\
 &  &  & 90 & 6.4 $\pm$ 1.4 & 93.5 & 35.23 & 6.8 $\pm$ 1.1 & 94.3 & 0.01  \\
\midrule
 &  &  & 100 & 8.9 $\pm$ 0.9 & 100 & 1.05 & 8.9 $\pm$ 0.9 & 100 & 1.20  \\
dermatology & 41 & 11.1 $\pm$ 1.2 & 95 & 7.5 $\pm$ 1.7 & 98.6 & 1.33 & 7.5 $\pm$ 1.7 & 98.6 & 0.00  \\
 &  &  & 90 & 7.4 $\pm$ 1.6 & 98.3 & 1.18 & 7.4 $\pm$ 1.6 & 98.3 & 0.00  \\
\midrule
 &  &  & 100 & 9.0 $\pm$ 1.1 & 100 & 2.85 & 9.0 $\pm$ 1.0 & 100 & 1.32  \\
kr-vs-kp & 86 & 10.9 $\pm$ 1.0 & 95 & 7.8 $\pm$ 2.0 & 97.6 & 5.16 & 7.5 $\pm$ 2.0 & 97.2 & 0.01  \\
 &  &  & 90 & 5.8 $\pm$ 1.7 & 91.6 & 4.92 & 5.6 $\pm$ 1.7 & 91.5 & 0.01  \\
\midrule
 &  &  & 100 & 8.9 $\pm$ 0.8 & 100 & 295.30 & 8.9 $\pm$ 0.8 & 100 & 1.36  \\
letter & 361 & 12.7 $\pm$ 1.4 & 95 & 8.7 $\pm$ 1.0 & 99.5 & 219.68 & 8.7 $\pm$ 0.9 & 99.6 & 0.01  \\
 &  &  & 90 & 8.4 $\pm$ 1.0 & 97.4 & 160.57 & 8.4 $\pm$ 0.9 & 97.5 & 0.01  \\
\midrule
 &  &  & 100 & 8.6 $\pm$ 1.1 & 100 & 5.50 & 8.6 $\pm$ 1.1 & 100 & 1.20  \\
soybean & 184 & 9.9 $\pm$ 1.7 & 95 & 8.5 $\pm$ 1.1 & 99.7 & 8.27 & 8.5 $\pm$ 1.1 & 99.7 & 0.00  \\
 &  &  & 90 & 7.9 $\pm$ 1.3 & 95.8 & 8.41 & 8.0 $\pm$ 1.3 & 96.3 & 0.00  \\
\midrule
 &  &  & 100 & 10.0 $\pm$ 0.3 & 100 & 6.56 & 10.1 $\pm$ 0.4 & 100 & 1.32  \\
spambase & 254 & 11.1 $\pm$ 0.5 & 95 & 5.1 $\pm$ 0.6 & 95.9 & 12.92 & 5.1 $\pm$ 0.8 & 96.8 & 0.01  \\
 &  &  & 90 & 3.1 $\pm$ 0.5 & 90.3 & 11.63 & 3.1 $\pm$ 0.6 & 90.4 & 0.02  \\
\midrule
 &  &  & 100 & 8.4 $\pm$ 0.7 & 100 & 13.80 & 8.4 $\pm$ 0.7 & 100 & 1.66  \\
texture & 175 & 8.8 $\pm$ 0.9 & 95 & 7.2 $\pm$ 1.0 & 98.9 & 18.02 & 7.3 $\pm$ 1.0 & 99.2 & 0.03  \\
 &  &  & 90 & 7.2 $\pm$ 0.9 & 98.5 & 31.23 & 7.2 $\pm$ 1.0 & 99.0 & 0.05  \\
%


\bottomrule[1.2pt]
\end{tabular}
}
\caption{ Assessing explanations of  $\mdrset$ and $\adrset$. 
	%
	(For each dataset, we run the explainers on instances that obtain 
	AXp's (i.e.\  $\drset$ s.t. $\delta = 1$)) of length greater than 7)	
	%
	%
	Column {\bf \#I} denotes the number of tested instances. 
	%randomly 
	%picked from the training data. 
	%
	Column {$\bm\delta$} reports in (\%) the value of the threshold  $\delta$.
	% 
	{\bf Path}   reports the average 
	 depth of paths consistent with the instances. 
	%
 	In column $\mdrset$ (resp.\ $\adrset$), column  {\bf Length} reports 
	the average length of the explanations, {\bf Precision} reports in (\%)  
	 the average precision (defined in (\ref{eq:drs})) of computed explanations 
	 and  column {\bf Time} reports in (sec)  the average runtime that takes 
	 the algorithm
	 to compute an explanation ($\pm$ denotes the standard deviation).
	%
	%{$\bm\drset$} shows the number in  (\%) of $\adrset$'s that are $\drset$'s. 
	%{\bf m$_{\bm\subseteq}$}	shows the number in  (\%) of $\adrset$'s that are 
	%subset-minimal, i.e.\  $\drset$'s. 
	 } 
\label{tab:paxp-res}
\end{table*}


==> tabs/dt/smtenc2.tex <==
\begin{table}[t]
  \centering
  \renewcommand{\arraystretch}{1.15}
  \renewcommand{\tabcolsep}{0.3575em}
  \scalebox{0.7}{
    \begin{tabular}{c|c|c|} \toprule
      Var.   & $R_4\cong{Q_1}$  & $R_5\cong{Q_2}$ \\
      \toprule
      $s_{1,0,k}$ & $s_{1,0,4}=0$ & $s_{1,0,5}=0$ 
      \\
      %
      $s_{1,1,k}$ &
      $s_{1,0,4}+\ite(u_1,\eta_{0,4},0)$ &
      $s_{1,0,5}$ 
      \\ 
      %
      $s_{1,2,k}$ &
      $s_{1,1,4}$ &
      $s_{1,1,5}+\ite(u_1,\eta_{0,5},0)$
      \\ 
      %
      $s_{1,3,k}$ &
      $s_{1,2,4}$ &
      $s_{1,2,5}+\ite(u_1,\eta_{0,5},0)$
      \\
      %
      $s_{1,4,k}$ &
      $s_{1,3,4}$ &
      $s_{1,3,5}+\eta_{0,5}$
      \\
      \midrule
      %
      $\eta_{1,k}$ & $s_{1,4,4}$ & $s_{1,4,5}$
      \\
      \midrule
      %
      $s_{2,0,k}$ & $s_{2,0,4}=0$ & $s_{2,0,5}=0$
      \\
      %
      $s_{2,1,k}$ &
      $s_{2,0,4}+\ite(u_2,\eta_{1,4},0)$ &
      $s_{2,0,5}+\ite(u_2,\eta_{1,5},0)$
      \\
      %
      $s_{2,2,k}$ &
      $s_{2,1,4}$ &
      $s_{2,1,5}$
      \\
      %
      $s_{2,3,k}$ &
      $s_{2,2,4}$ &
      $s_{2,2,5}$
      \\
      %
      $s_{2,4,k}$ &
      $s_{2,3,4}$ &
      $s_{2,3,5}$
      \\
      \midrule
      %
      $\eta_{2,k}$ &  $s_{2,4,4}$ & $s_{2,4,5}$
      \\
      \midrule
      %
      $s_{3,0,k}$ & $s_{3,0,4}=0$ & $s_{3,0,5}=0$
      \\
      %
      $s_{3,1,k}$ &
      $s_{3,0,4}+\ite(u_3,\eta_{2,4},0)$ &
      $s_{3,0,5}+\ite(u_3,\eta_{2,5},0)$
      \\
      %
      $s_{3,2,k}$ &
      $s_{3,1,4}+\eta_{2,4}$ &
      $s_{3,1,5}$
      \\
      \midrule
      %
      $\eta_{3,k}$ & $s_{3,2,4}$ & $s_{3,2,5}$
      \\
      \bottomrule
    \end{tabular}
  }
  \caption{Partial addition-based SMT encoding for paths with
    prediction $\ominus$, with $(\mbf{v},c)=((4,4,2),\oplus)$,
    and with $\eta_{0,4}=\eta_{0,5}=1$} \label{tab:smtenc2}
\end{table}


==> tabs/nbc/ex02a.tex <==
%
\begin{tabular}{|c|ccccc|c|} \toprule
  & $\prob(a)$ & $\prob(r_1|a)$ & $\prob(\neg{r_2}|a)$ & $\prob(r_3|a)$
  & $\prob(\neg{r_4}|a)$ & $\nu(a)$
  \\ \midrule
  %
  $\prob(\cdot)$ & 0.10 & 0.95 & 0.95 & 0.02 & 0.80 &
  \\
  %
  $\lprob(\cdot)$ & 1.70 & 3.95 & 3.95 & 0.09 & 3.78 & 13.47
  \\ \bottomrule
\end{tabular}


==> tabs/nbc/ex02b.tex <==
%
\begin{tabular}{|c|ccccc|c|} \toprule
  & $\prob(\neg{a})$ & $\prob(r_1|\neg{a})$ &
  $\prob(\neg{r_2}|\neg{a})$ & $\prob(r_3|\neg{a})$ &
  $\prob(\neg{r_4}|\neg{a})$ & $\nu(\neg{a})$ 
  \\ \midrule
  %
  $\prob(\cdot)$ & 0.90 & 0.03 & 0.18 & 0.34 & 0.08 &
  \\
  %
  $\lprob(\cdot)$ & 3.89 & 0.49 & 2.29 & 2.92 & 1.47 & 11.06
  \\ \bottomrule
\end{tabular}


==> tabs/nbc/ex03.tex <==
\renewcommand{\tabcolsep}{0.575em}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{|c|cccccc||c|cccccc|} \hline
  $w_0^{\oplus}$ &
  $v^{\oplus}_{0,1}$ & $v^{\oplus}_{1,1}$ &
  $v^{\oplus}_{0,2}$ & $v^{\oplus}_{1,2}$ &
  $v^{\oplus}_{0,3}$ & $v^{\oplus}_{1,3}$ &
  %
  $w_0^{\ominus}$ &
  $v^{\ominus}_{0,1}$ & $v^{\ominus}_{1,1}$ &
  $v^{\ominus}_{0,2}$ & $v^{\ominus}_{1,2}$ &
  $v^{\ominus}_{0,3}$ & $v^{\ominus}_{1,3}$
  \\ \hline
  25 &
  15 & 15 &
  15 & 30 &
  20 & 25 &
  %
  35 &
  15 & 20 &
  20 & 10 &
  10 & 20
  \\ \hline
\end{tabular}


==> tabs/nbc/ex04.tex <==
\renewcommand{\tabcolsep}{0.425em}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{|c|cccccccc||c|cccccccc|} \hline
  $w_0^{\oplus}$ &
  $v^{\oplus}_{0,1}$ & $v^{\oplus}_{1,1}$ &
  $v^{\oplus}_{0,2}$ & $v^{\oplus}_{1,2}$ &
  $v^{\oplus}_{0,3}$ & $v^{\oplus}_{1,3}$ &
  $v^{\oplus}_{0,4}$ & $v^{\oplus}_{1,4}$ &
  %
  $w_0^{\ominus}$ &
  $v^{\ominus}_{0,1}$ & $v^{\ominus}_{1,1}$ &
  $v^{\ominus}_{0,2}$ & $v^{\ominus}_{1,2}$ &
  $v^{\ominus}_{0,3}$ & $v^{\ominus}_{1,3}$ &
  $v^{\ominus}_{0,4}$ & $v^{\ominus}_{1,4}$
  \\ \hline
  1.70 &
  1.00 & 3.95 &
  3.95 & 1.00 &
  3.98 & 0.09 &
  3.78 & 2.39 &
  %
  3.89 &
  3.97 & 0.49 &
  2.29 & 3.80 &
  0.58 & 2.92 &
  1.47 & 3.92
  \\ \hline
\end{tabular}


==> tabs/nbc/ex06e.tex <==
\begin{table*}[tb]
  \begin{center}
    \renewcommand{\arraystretch}{0.9}
    \renewcommand{\tabcolsep}{0.4em}
    \begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
      \diagbox{$k$}{$r$} 
      & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16
      \\ \hline\hline
      %
1 & \textemdash & 0 & 1 & \textemdash & 1 & 1 & \textemdash & 1 & 1 & \textemdash & 1 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash\\
\hline
2 & \textemdash & \textemdash & 0 & 1 & \textemdash & 1 & 1 & \textemdash & 1 & 1 & \textemdash & 1 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash\\
\hline
3 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 1 & \textemdash & 1 & \textemdash & \textemdash & \textemdash & 2 & \textemdash & 2 & \textemdash & \textemdash\\
\hline
4 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 2 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 4 & \textemdash\\
\hline
5 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 6\\
\hline
      %
    \end{tabular}
    \caption{DP table for $\fml{S} = \{1, 2\}$ (Example~\ref{ex:06})} \label{tab:ex06e}
  \end{center}
\end{table*}


==> tabs/nbc/ex06g.tex <==
\begin{table*}[tb]
  \begin{center}
    \renewcommand{\arraystretch}{0.9}
    \renewcommand{\tabcolsep}{0.4em}
    \begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}\hline
      \diagbox{$k$}{$r$} 
      & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16
      \\ \hline\hline
      %
1 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 1 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash\\
\hline
2 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 1 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash\\
\hline
3 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 1 & \textemdash & \textemdash\\
\hline
4 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 1 & \textemdash\\
\hline
5 & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & \textemdash & 1\\
\hline
      %
    \end{tabular}
    \caption{DP table for $\fml{S} = \{0, 1, 2, 3, 4, 5\}$ (Example~\ref{ex:06})} \label{tab:ex06g}
  \end{center}
\end{table*}


==> tabs/nbc/paxp-len7.tex <==
\setlength{\tabcolsep}{5pt}
\let\lpr\undefined
\let\rpr\undefined
\newcommand{\lpr}{(}
\newcommand{\rpr}{)}



\begin{table*}[t]
\centering
\resizebox{0.75\textwidth}{!}{
  \begin{tabular}{l >{\lpr}S[table-format=2,table-space-text-pre=\lpr]S[table-format=1,table-space-text-post=\rpr]<{\rpr}
  			 S[table-format=2.2] S[table-format=3]  c c c  S[table-format=1.3]  }
\toprule[1.2pt]
\multirow{2}{*}{\bf Dataset} & \multicolumn{2}{c}{\multirow{2}{*}{\bf (\#F~~~~~~\#C)}}  &  {\bf NBC}  &  & {\bf AXp}  &   \multicolumn{3}{c}{\bf PAXp}  \\
\cmidrule[0.8pt](lr{.75em}){4-4}
\cmidrule[0.8pt](lr{.75em}){6-6}
\cmidrule[0.8pt](lr{.75em}){7-9}
 & \multicolumn{2}{c}{}  & {\bf A\%} & {\bf \#I} & {\bf Length}  &  {\bf Length} & {\bf Precision} & {\bf Time} \\  

\toprule[1.2pt]

adult & 13 & 2 & 81.37 & 200 & 6.85$\pm$ 1.15 & 5.3 $\pm$ 1.13 & 98.62 $\pm$ 0.46 & 0.026 \\
\midrule
agaricus\_lepiota & 23 & 2 & 95.41 & 200 & 10.34$\pm$ 2.53 & 7.6 $\pm$ 1.45 & 97.30 $\pm$ 3.53 & 0.508 \\
\midrule
chess & 37 & 2 & 88.34 & 200 & 12.11$\pm$ 3.74 & 5.1 $\pm$ 3.80 & 82.15 $\pm$ 22.19 & 2.327 \\
\midrule
dermatology & 35 & 6 & 99.66 & 147 & 9.28$\pm$ 1.64 & 6.0 $\pm$ 1.19 & 98.40 $\pm$ 1.13 & 1.399 \\
\midrule
house-votes-84 & 17 & 2 & 89.66 & 81 & 5.31$\pm$ 1.43 & 4.3 $\pm$ 1.44 & 98.90 $\pm$ 0.32 & 0.014 \\
\midrule
kr-vs-kp & 37 & 2 & 88.07 & 200 & 12.24$\pm$ 3.85 & 5.5 $\pm$ 3.81 & 80.25 $\pm$ 24.59 & 2.553 \\
\midrule
lymphography & 19 & 4 & 88.98 & 60 & 8.82$\pm$ 0.88 & 7.4 $\pm$ 0.82 & 98.67 $\pm$ 0.45 & 0.052 \\
\midrule
mushroom & 23 & 2 & 95.51 & 200 & 10.71$\pm$ 2.33 & 7.7 $\pm$ 1.26 & 97.56 $\pm$ 2.89 & 0.481 \\
\midrule
threeOf9 & 10 & 2 & 83.13 & 103 & 4.22$\pm$ 0.42 & 4.1 $\pm$ 0.59 & 99.79 $\pm$ 0.54 & 0.002 \\
\midrule
xd6 & 10 & 2 & 81.36 & 176 & 4.55$\pm$ 0.89 & 3.8 $\pm$ 1.34 & 98.86 $\pm$ 0.70 & 0.002 \\

\bottomrule[1.2pt]
\end{tabular}
}
\caption{ Assessing PAXp explanations for NBCs. 
	%	
	Columns {\bf \#F} and  {\bf \#C} show, respectively, number of features and 
	classes in the Dataset.
	%
	 Column {\bf A\%} reports in (\%) the training accuracy of the classifier. 
	 %
	 Column {\#I} reports the number of tested instances.
	 %
	 %Column {$\delta$} reports in (\%) the used value of the parameter $\delta$.
	 %
	 Columns {\bf Length} and {\bf Precision} report, respectively, the average  
	 explanation length and the average explanation precision ($\pm$ denotes 
	 the standard  deviation). 
	 %
	 Finally, the average runtime  to compute an explanation is shown 
	 (in seconds) in {\bf Time}.
	 } 
\label{tab:paxp-len7}
\end{table*}


==> tango.tex <==
% tango colors
%
% yellow
\definecolor{tyellow1}{HTML}{FCE94F}
\definecolor{tyellow2}{HTML}{EDD400}
\definecolor{tyellow3}{HTML}{C4A000}
%
% orange
\definecolor{torange1}{HTML}{FCAF3E}
\definecolor{torange2}{HTML}{F57900}
\definecolor{torange3}{HTML}{C35C00}
%
% brown
\definecolor{tbrown1}{HTML}{E9B96E}
\definecolor{tbrown2}{HTML}{C17D11}
\definecolor{tbrown3}{HTML}{8F5902}
%
% green
\definecolor{tgreen1}{HTML}{8AE234}
\definecolor{tgreen2}{HTML}{73D216}
\definecolor{tgreen3}{HTML}{4E9A06}
%
% blue
\definecolor{tblue1}{HTML}{729FCF}
\definecolor{tblue2}{HTML}{3465A4}
\definecolor{tblue3}{HTML}{204A87}
%
% purple
\definecolor{tpurple1}{HTML}{AD7FA8}
\definecolor{tpurple2}{HTML}{75507B}
\definecolor{tpurple3}{HTML}{5C3566}
%
% red
\definecolor{tred1}{HTML}{EF2929}
\definecolor{tred2}{HTML}{CC0000}
\definecolor{tred3}{HTML}{A40000}
%
% light gray
\definecolor{tlgray1}{HTML}{EEEEEC}
\definecolor{tlgray2}{HTML}{D3D7CF}
\definecolor{tlgray3}{HTML}{BABDB6}
%
% dark gray
\definecolor{tdgray1}{HTML}{888A85}
\definecolor{tdgray2}{HTML}{555753}
\definecolor{tdgray3}{HTML}{2E3436}

